Stabilization of the fluidic pinball with gradient-enriched machine learning control

We stabilize the flow past a cluster of three rotating cylinders, the fluidic pinball, with automated gradient-enriched machine learning algorithms. The control laws command the rotation speed of each cylinder in an open- and closed-loop manner. These laws are optimized with respect to the average distance from the target steady solution in three successively richer search spaces. First, stabilization is pursued with steady symmetric forcing. Second, we allow for asymmetric steady forcing. And third, we determine an optimal feedback controller employing nine velocity probes downstream. As expected, the control performance increases with every generalization of the search space. Surprisingly, both open- and closed-loop optimal controllers include an asymmetric forcing, which surpasses symmetric forcing. Intriguingly, the best performance is achieved by a combination of phasor control and asymmetric steady forcing. We hypothesize that asymmetric forcing is typical for pitchfork bifurcated dynamics of nominally symmetric configurations. Key enablers are automated machine learning algorithms augmented with gradient search: explorative gradient method for the open-loop parameter optimization and a gradient-enriched machine learning control (gMLC) for the feedback optimization. gMLC learns the control law significantly faster than previously employed genetic programming control. The gMLC source code is freely available online.

==> App1.tex <==
\section{Optimal periodic forcing} \label{appA}
In this appendix we aim to stabilize the symmetric steady solution thanks to a symmetric periodic forcing.
In this case, the two back cylinders oscillating in opposite directions whereas the front cylinder stays still.
The control ansatz is the following:
\begin{equation*}
\begin{array}{cc}
b_1 = & 0 \\
b_2 = &  ~B \cos (2\pi F t) \\
b_2 = & -B \cos (2\pi F t)
\end{array}
\end{equation*}
with $B$, the amplitude of the oscillations, and $F$, the frequency, being the two parameter to optimize.
The search space is limited to $(B,F/f_1) \in [0;5]\times[0;10]$ as higher amplitudes and frequencies would be beyond our solver capabilities.
This two-dimensional search space is explored with EGM.
The contour plot in figure~\ref{fig:EGMPeriodicMap} depicts the search space based on $J_a/J_0$ and $J_b$.
The contour plot has been produced thanks to simulations for $B =[0.1,0.5,1,2,3.5,5]$ and $F/f_1=[0.1,0.5,1,2,3.5,5,7.5,10]$.
The steps were finer for low frequencies and low amplitudes.
The individuals have been evaluated over 250 convective time units.
We notice that there is only one minimum on the plane, close to $(B,F/f_1) = (3.5,3.5)$.
Also, forcing at frequency close to the natural frequency resonates with the flow and increases drastically the distance to the steady solution for high amplitudes.
For $J_b$, the contour map tends towards a high plateau at high frequencies and amplitudes.
The three initial control laws for EGM are the center of the box and increments of 1/5 of the box in each direction: $(2.5,5)$, $(3,5)$, $(2.5,6)$.
Just as expected, the exploration steps (LHS in blue) spreads rather evenly on the plane whereas the exploitation steps (\textrm{simplex} in yellow) quickly falls into the global minimum.

%% Ja, Jb maps
\begin{figure}
\centering
%
\begin{subfigure}{.45\textwidth}
  \centering
\includegraphics[width=\linewidth]{Figures/Perio/EGM_Pinball_Period}
\caption{\label{fig:EGM_periodic_ja}$J_a/J_0$.}
\end{subfigure}%
%
\hfil
%
\begin{subfigure}{.45\textwidth}
  \centering
\includegraphics[width=1.\textwidth]{Figures/Perio/EGM_Pinball_Period_Jb}
\caption{\label{fig:EGM_periodic_jb}$J_b$.}
\end{subfigure}
  \caption{Contour plot for $J_a/J_0$ (a) and $J_b$ (b) as a function of the amplitude $B$ and the reduced frequency $F/f_1$. For (a), blue regions denote good perfomances, white denote costs that are equivalent to the natural flow and red regions denote bad performances. For (b), the color code describes the energy consumption. 
  The white zone on the bottom left is due to the limits of our simulation capabilities.
  The dots represent the individuals tested with EGM: black diamond for the initial conditions, blue for the exploration steps and yellow for the exploitation steps.}
\label{fig:EGMPeriodicMap}
\end{figure}

%% Pareto diagram
%\begin{figure}
%  \centerline{\includegraphics[width=0.75\linewidth]{Figures//Perio/PeriodicParetoDiagram}}
%  \caption{Pareto diagram for the periodic forcing }
%\label{fig:ParetoPeriodic}
%\end{figure}
Figure~\ref{fig:Perioprog} shows the progression of the best individual throughout the evaluations.
The optimization process lasted 25 cycles during which EGM converges rather quickly as $J_a/J_0$, the amplitude and the frequecy reach asymptotic values, without any significant improvement afterwards.
The parameters of the best symmetric periodic forcing are then:
\begin{equation*}
\begin{array}{cc}
B_{EGM} = 3.51\\
F_{EGM} / f_1= 3.19
\end{array}
\end{equation*}
%% Progression
\begin{figure}
\centering
%
\begin{subfigure}{.45\textwidth}
  \centering
\includegraphics[width=1.\textwidth]{Figures/Perio/AmpFreqProgression}
\caption{\label{fig:AmpFreqprog}}
\end{subfigure}%
%
\hfil
%
\begin{subfigure}{.45\textwidth}
  \centering
\includegraphics[width=1.\textwidth]{Figures/Perio/JPeriodProg}
\caption{\label{fig:JPerioprog}}
\end{subfigure}%
\caption{\label{fig:Perioprog}Evolution of (a) the amplitude and the frequency and (b) the reduced cost $J_a/J_0$ as a function of the number of evaluations $i$, for the EGM optimization process.
The red line on (b) shows the evolution of the best cost.
The evaluation time is 250 convective time units.}
\label{fig:fig}
\end{figure}
The proximity between the initial values and the aimed minimum certainly accelerates the observed convergences.
Figure~\ref{fig:EGM_Perio_characteristics} show the evolution of the lift coefficient, the phase portrait, the power spectral density and the instantaneous cost function $j_a$ for the controlled flow.
The lift coefficient presents rather symmetric low amplitude oscillations, see figure~\ref{fig:CL_Perio}.
This goes along with the flow symmetry in figure~\ref{fig:EGM_Perio_T1}-\ref{fig:EGM_Perio_T8}.
The oscillations are explained by the remaining vortex shedding on both the upper and lower side of the fluidic pinball.
Even though the far field is close to the symmetric steady solution, this periodic solution changes radically the near field profile.
The near jet is completely flattened. 
We can identify parts of the two vorticity branches close to the cylinders in figure~\ref{fig:EGM_Perio_T3}, \ref{fig:EGM_Perio_T4} and \ref{fig:EGM_Perio_T5}.
Moreover the vorticity around the cylinders is more intense compared to the initial steady solution.
This difference is present in the final mean value $j_a$ in figure~\ref{fig:DSS_Perio} and is responsible for the high actuation power expanse, $J_b=4.51$.
The phase portrait shows a periodic regime regime, though deformed by the harmonics.
The mean frequency $f_7=0.398$ is slightly lower than the forcing frequency $F_{EGM} = 0.37$ and much lower than the natural frequency, showing that it is not just a simple frequency locking, but a nonlinear frequency crosstalk.
The non centered phase portrait indicates that there is still an asymmetry in the flow, that may be a residual effect of the grid's asymmetry.
The mean field in figure~\ref{fig:Mean_EGM_Perio} is similar to the symmetric steady solution, however the near jet complety vanished, in addition, the distance between the upper and lower vorticity branches is wider compared to the symmetric steady solution.
%% Figures : EGM Periodic flow characteristics
\begin{figure}
\centering
%
\begin{subfigure}{.45\textwidth}
  \centering
\includegraphics[width=1.\textwidth]{Figures/Perio/Cl_EGM_Perio}
\caption{\label{fig:CL_Perio}}
\end{subfigure}%
%
\hfil
%
\begin{subfigure}{.45\textwidth}
  \centering
\includegraphics[width=1.\textwidth]{Figures/Perio/PP_EGM_Perio}
\caption{\label{fig:PP_Perio}}
\end{subfigure}

%
\begin{subfigure}{.45\textwidth}
  \centering
\includegraphics[width=1.\textwidth]{Figures/Perio/DSS_EGM_Perio}
\caption{\label{fig:PSD_Perio}}
\end{subfigure}%
%
\hfil
%
\begin{subfigure}{.45\textwidth}
  \centering
\includegraphics[width=1.\textwidth]{Figures/Perio/PSD_EGM_Perio}
\caption{\label{fig:DSS_Perio}}
\end{subfigure}
\caption{\label{fig:EGM_Perio_characteristics}Characteristics of the best periodic forcing found with EGM. (a) Time evolution of the lift coefficient $C_L$, (b) phase portrait (c) time evolution of instantaneous cost function $j_a$ and (d) Power Spectral Density (PSD).
The control starts at $t=400$.
The unforced phase is depicted in blue and the forced one in red.
The phase portrait and the PSD are computed over $t \in [900,1400]$, during the permanent regime.}
\end{figure}


% % gMLC flow snapshots
\begin{figure}
\centering
%
\begin{subfigure}{.45\textwidth}
  \centering
\includegraphics[width=1.\textwidth]{Figures/Snapshots/EGM_Perio_T1}
\caption{\label{fig:EGM_Perio_T1}$t+T_7/8$}
\end{subfigure}%
%
\hspace{0.5cm}
%
\begin{subfigure}{.45\textwidth}
  \centering
\includegraphics[width=1.\textwidth]{Figures/Snapshots/EGM_Perio_T2}
\caption{\label{fig:EGM_Perio_T2}$t+2T_7/8$}
\end{subfigure}

\begin{subfigure}{.45\textwidth}
  \centering
\includegraphics[width=1.\textwidth]{Figures/Snapshots/EGM_Perio_T3}
\caption{\label{fig:EGM_Perio_T3}$t+3T_7/8$}
\end{subfigure}%
%
\hspace{0.5cm}
%
\begin{subfigure}{.45\textwidth}
  \centering
\includegraphics[width=1.\textwidth]{Figures/Snapshots/EGM_Perio_T4}
\caption{\label{fig:EGM_Perio_T4}$t+4T_7/8$}
\end{subfigure}

\begin{subfigure}{.45\textwidth}
  \centering
\includegraphics[width=1.\textwidth]{Figures/Snapshots/EGM_Perio_T5}
\caption{\label{fig:EGM_Perio_T5}$t+5T_7/8$}
\end{subfigure}%
%
\hspace{0.5cm}
%
\begin{subfigure}{.45\textwidth}
  \centering
\includegraphics[width=1.\textwidth]{Figures/Snapshots/EGM_Perio_T6}
\caption{\label{fig:EGM_Perio_T6}$t+6T_7/8$}
\end{subfigure}

\begin{subfigure}{.45\textwidth}
  \centering
\includegraphics[width=1.\textwidth]{Figures/Snapshots/EGM_Perio_T7}
\caption{\label{fig:EGM_Perio_T7}$t+7T_7/8$}
\end{subfigure}%
%
\hspace{0.5cm}
%
\begin{subfigure}{.45\textwidth}
  \centering
\includegraphics[width=1.\textwidth]{Figures/Snapshots/EGM_Perio_T8}
\caption{\label{fig:EGM_Perio_T8}$t+T_7$}
\end{subfigure}

\begin{subfigure}{.45\textwidth}
  \centering
\includegraphics[width=1.\textwidth]{Figures/Snapshots/SteadySolution}
\caption{Symmetric steady solution}
\end{subfigure}%
%
\hspace{0.5cm}
%
\begin{subfigure}{.45\textwidth}
  \centering
\includegraphics[width=1.\textwidth]{Figures/Snapshots/Mean_EGM_Perio}
\caption{\label{fig:Mean_EGM_Perio}Mean field}
\end{subfigure}
\caption{\label{fig:EGM_Periosnap}
Vorticity fields of the best periodic forcing found with EGM. (a)-(f) Time evolution of the vorticity field throughout the last period of the 1400 convective time units simulation, (i) the objective symmetric steady solution and (j) the mean field of the forced flow.
The color code is the same as figure~\ref{fig:unforced_flow}.
$T_6$ is the period associated to the frequency $f_6$.
The mean field is computed by averaging 200 periods.}
\end{figure}
